P-Tuning v2: Prompt Tuning Can Be Comparable to Fine-tuning Universally Across Scales and Tasks

Prompt tuning, which only tunes continuous prompts with a frozen language model, substantially reduces per-task storage and memory usage at training. However, in the context of NLU, prior work reveals that prompt tuning does not perform well for normal-sized pretrained models. We also find that existing methods of prompt tuning cannot handle hard sequence labeling tasks, indicating a lack of universality. We present a novel empirical finding that properly optimized prompt tuning can be universally effective across a wide range of model scales and NLU tasks. It matches the performance of finetuning while having only 0.1%-3% tuned parameters. Our method P-Tuning v2 is an implementation of Deep Prompt Tuning \cite{li2021prefix,qin2021learning} optimized and adapted for NLU. Given the universality and simplicity of P-Tuning v2, we believe it can serve as an alternative to finetuning and a strong baseline for future research.Our code and data are released at https://github.com/THUDM/P-tuning-v2.

==> 2_related.tex <==
\section{Related Work} \label{sec:related}
% \section{Related Work}

\vpara{Prompting.}
Prompting~\cite{liu2021pre} refers to leverage special templates in input to aid language model's prediction on both understanding and generation. Recently, various prompting strategies including discrete natural language prompt~\cite{shin2020autoprompt,gao2020making}, continuous prompts~\cite{liu2021gpt,li2021prefix,lester2021power,qin2021learning,zhong2021factual}, tuning bias~\cite{logan2021cutting} and many other prompting strategies have appeared. 

Prompting's effectiveness in many NLP applications has been verified in recent literature, including text classification~\cite{hu2021knowledgeable,min2021noisy}, entity typing~\cite{ding2021prompt}, few-shot learning~\cite{zheng2021fewnlu,xu2021fewclue}, relation extraction~\cite{chen2021adaprompt,han2021ptr}, knowledge probing~\cite{zhong2021factual}, named entity recognition~\cite{chen2021lightner}, machine translation~\cite{tan2021msp,wang2021language} and dialogue system~\cite{wang2021topicrefine}.

In this work, we are especially interested in scaling prompting methods to smaller models and hard sequence NLU tasks.

==> tables/ner.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \renewcommand\tabcolsep{4.0pt}
    %\ra{1.2}
    \begin{tabular}{@{}
    l p{0.7cm}<{\raggedright} 
    p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.9cm}<{\centering} c 
    p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.9cm}<{\centering} c 
    p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.9cm}<{\centering}
    @{}} \toprule[1.5pt]
    
                        &\multirow{2}{*}{\#Size}& \multicolumn{4}{c}{CoNLL03}   & \phantom{} & \multicolumn{4}{c}{OntoNotes 5.0} & \phantom{} & \multicolumn{4}{c}{CoNLL04}   \\
                        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16}
                        && FT    & PT & PT-2 & MPT-2     && FT    & PT & PT-2 & MPT-2    && FT    & PT & PT-2 & MPT-2    \\
                        \midrule[1.2pt]
    BERT$_{\rm large}$   & 335M & \best 92.8   & 81.9 & 90.2  & \secbest 91.0 && \best 89.2  & 74.6 & \secbest 86.4  & 86.3       && \secbest 85.6  & 73.6 & 84.5  & \best 86.6    \\
    RoBERTa$_{\rm large}$& 355M & 92.6   & 86.1 & \secbest 92.7  & \best 92.8 && \best 89.8  & 80.8 & \secbest 89.4  & \best89.8       && \secbest 88.8  & 76.2 & 87.8  & \best90.6    \\
    DeBERTa$_{\rm xlarge}$&750M & \best 93.1   & 90.2 & \best 93.1  & \best 93.1 && \secbest 90.4  & 85.1 & \secbest 90.4  & \best 90.5       && \secbest 89.1  & 82.4 & 86.5  & \best 90.1    \\
    \bottomrule[1.5pt]
    \end{tabular}
    \caption{Results on Named Entity Recognition (NER) test set (all metrics are micro-f1 score). P-tuning v2 is generally comparable to fine-tuning, and multitask P-tuning v2 can bring in a further improvement. (FT: fine-tuning; PT: P-tuning \& \citet{lester2021power}; PT-2: P-tuning v2; MPT-2: Multi-task P-tuning v2)}
    \label{tab:ner}
\end{table*}

==> tables/nlu.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \renewcommand\tabcolsep{3.0pt}
    %\ra{1.2}
    \begin{tabular}{@{}
    l p{0.7cm}<{\raggedright}
    p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.7cm}<{\centering} c
    p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.7cm}<{\centering}
    @{}} \toprule[1.5pt]
                        &\multirow{3}{*}{\#Size}& \multicolumn{6}{c}{GLUE dev}   & \phantom{} & \multicolumn{9}{c}{SuperGLUE dev} \\
                        \cmidrule{3-8} \cmidrule{10-18} 
                        && \multicolumn{3}{c}{SST-2}    & \multicolumn{3}{c}{MNLI-m} && \multicolumn{3}{c}{RTE} & \multicolumn{3}{c}{BoolQ}     & \multicolumn{3}{c}{CB}    \\
                        && FT   & PT    & PT-2    & FT    & PT    & PT-2    && FT    & PT    & PT-2    & FT    & PT    & PT-2    & FT    & PT    & PT-2  \\
                        \midrule[1.2pt]
    BERT$_{\rm large}$   & 335M & \secbest 93.2  & 92.4  & \best 93.6  & \best 86.6  & 75.6 & \secbest 85.8  && \secbest 70.4    & 53.5  & \best 78.3  & \best 77.7 & 67.2 & \secbest 75.8  & \best 94.6 & 80.4 & \best 94.6 \\
    RoBERTa$_{\rm large}$& 355M & \best 96.4  & 95.3 & \secbest 96.3  & \secbest 90.2  & 83.8 & \best 90.4  && \secbest 86.6    & 58.8  &\best  88.4  & \best 86.9 & 62.3 & \secbest 84.8  & \secbest 98.2 & 71.4 & \best 100 \\
    \midrule
    GLM$_{\rm xlarge}$   & 2B   & - & - & - & - & - & - && \best 90.3 & \secbest 85.6 & \best 90.3 & \best 88.3 & 79.7 & \secbest 87.0 & \best 96.4 & \secbest 76.4 & \best 96.4\\
    GLM$_{\rm xxlarge}$  & 10B  & - & - & - & - & - & - && \best 93.1 & \secbest 89.9 & \best 93.1 & \secbest 88.7 & \best 88.8 & \best 88.8 & \best 98.7 & \secbest 98.2 & 96.4 \\
    \bottomrule[1.5pt]
    \end{tabular}
    \caption{Results on part of GLUE and SuperGLUE development set (all metrics are Accuracy). P-tuning v2 significantly surpasses P-tuning \& \citet{lester2021power} on models smaller than 10B and matches the performance of fine-tuning. (FT: fine-tuning; PT: P-tuning \& \citet{lester2021power}; PT-2: P-tuning v2). }
    \label{tab:nlu}
\end{table*}

==> tables/qa.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \renewcommand\tabcolsep{3.0pt}
    %\ra{1.2}
    \begin{tabular}{@{}
    l p{0.7cm}<{\raggedright}
    p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering} c
    p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}p{0.6cm}<{\centering}
    @{}} \toprule[1.5pt]
                        &\multirow{3}{*}{\#Size}& \multicolumn{8}{c}{SQuAD 1.1 dev}   & \phantom{} & \multicolumn{8}{c}{SQuAD 2.0 dev} \\
                        \cmidrule{3-10} \cmidrule{12-19} 
                        && \multicolumn{2}{c}{FT}    & \multicolumn{2}{c}{PT} & \multicolumn{2}{c}{PT-2} & \multicolumn{2}{c}{MPT-2}     && \multicolumn{2}{c}{FT}    & \multicolumn{2}{c}{PT} & \multicolumn{2}{c}{PT-2} & \multicolumn{2}{c}{MPT-2}    \\
                        && EM   & F1    & EM    & F1    & EM    & F1    & EM    & F1    && EM   & F1    & EM    & F1    & EM    & F1    & EM    & F1    \\
                        \midrule[1.2pt]
    BERT$_{\rm large}$   & 335M & \best 84.2  & \best 91.1  & 1.0  & 8.5  & 77.8  & 86.0  & \secbest 82.3  & \secbest 89.6  && \best 78.7  & \best 81.9  & 50.2  & 50.2  & 69.7  & 73.5  & \secbest 72.7  & \secbest 75.9  \\
    RoBERTa$_{\rm large}$& 355M & \best 88.9  & \best 94.6  & 1.2  & 12.0 & \secbest 88.1  & \secbest 94.1  & 88.0  & \secbest 94.1  && \best 86.5  & \best 89.4  & 50.2  & 50.2  & 82.1  & 85.5  & \secbest 83.4  & \secbest 86.7  \\
    DeBERTa$_{\rm xlarge}$&750M & \secbest 90.1  & \secbest 95.5  & 2.4 & 19.0 & \best 90.4  & \best 95.7  & 89.6  & 95.4  && \secbest 88.3  & \secbest 91.1  & 50.2  & 50.2  & \best 88.4  & \best 91.1  & 88.1  & 90.8  \\
    \bottomrule[1.5pt]
    \end{tabular}
    \caption{Results on Question Answering (Extractive QA). Prompt tuning \& P-tuning performs extremely poor on question answering, while P-tuning v2's performance is generally reasonable, and can be better than fine-tuning with DeBERTa-xlarge. (FT: fine-tuning; PT: P-tuning \& \citet{lester2021power}; PT-2: P-tuning v2; MPT-2: Multi-task P-tuning v2)}
    \label{tab:qa}
\end{table*}

==> tables/srl.tex <==
\begin{table*}[t]
    \footnotesize
    \centering
    \renewcommand\tabcolsep{4.0pt}
    %\ra{1.2}
    \begin{tabular}{@{}
    l p{0.7cm}<{\raggedright} 
    p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.9cm}<{\centering} c 
    p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.9cm}<{\centering} c 
    p{0.6cm}<{\centering}p{0.7cm}<{\centering}p{0.7cm}<{\centering}p{0.9cm}<{\centering}
    @{}} \toprule[1.5pt]
                        &\multirow{2}{*}{\#Size}& \multicolumn{4}{c}{CoNLL12}   & \phantom{} & \multicolumn{4}{c}{CoNLL05 WSJ} & \phantom{} & \multicolumn{4}{c}{CoNLL05 Brown}   \\
                        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16}
                        && FT    & PT & PT-2 & MPT-2     && FT    & PT & PT-2 & MPT-2    && FT    & PT & PT-2 & MPT-2    \\
                        \midrule[1.2pt]
    BERT$_{\rm large}$   & 335M & \secbest 84.9   & 64.5. & 83.2 & \best 85.1 && \best 88.5  & 76.0  & \secbest 86.3  & \best 88.5       && \secbest 82.7  & 70.0& 80.7  & \best 83.1    \\
    RoBERTa$_{\rm large}$& 355M & \best 86.5   & 67.2  & 84.6  & \secbest 86.2 && \best 90.2  & 76.8  & 88.3  & \secbest 90.0       && \secbest 85.6  & 70.7  & 84.2  & \best 85.7    \\
    DeBERTa$_{\rm xlarge}$&750M & \secbest 86.5   & 74.1  & 85.7  & \best 87.1 && \best 91.2  & 82.3  & 90.6  & \secbest 91.1       && \secbest 86.9  & 77.7  & 86.3  & \best 87.3    \\
    \bottomrule[1.5pt]
    \end{tabular}
    \caption{Results on Semantic Role Labeling (SRL). P-tuning v2 shows a consistent improvement over \citet{lester2021power} \& P-tuning on SRL. (FT: fine-tuning; PT: P-tuning \& \citet{lester2021power}; PT-2: P-tuning v2; MPT-2: Multi-task P-tuning v2)}
    \label{tab:srl}
\end{table*}
